TrustMH-Bench: A Comprehensive Benchmark for Evaluating the Trustworthiness of Large Language Models in Mental Health

While Large Language Models (LLMs) demonstrate significant potential in providing accessible mental health support, their practical deployment raises critical trustworthiness concerns due to the domains high-stakes and safety-sensitive nature. Existing evaluation paradigms for general-purpose LLMs fail to capture mental health-specific requirements, highlighting an urgent need to prioritize and enhance their trustworthiness. To address this, we propose TrustMH-Bench, a holistic framework designed to systematically quantify the trustworthiness of mental health LLMs. By establishing a deep mapping from domain-specific norms to quantitative evaluation metrics, TrustMH-Bench evaluates models across eight core pillars: Reliability, Crisis Identification and Escalation, Safety, Fairness, Privacy, Robustness, Anti-sycophancy, and Ethics. We conduct extensive experiments across six general-purpose LLMs and six specialized mental health models. Experimental results indicate that the evaluated models underperform across various trustworthiness dimensions in mental health scenarios, revealing significant deficiencies. Notably, even generally powerful models (e.g., GPT-5.1) fail to maintain consistently high performance across all dimensions. Consequently, systematically improving the trustworthiness of LLMs has become a critical task. Our data and code are released.

==> tables/ap_psyethic_14_dataset.tex <==
\providecommand{\cellml}{\cellcolor[HTML]{F5E9DD}}
\providecommand{\cellmr}{\cellcolor[HTML]{D8DDD6}}
\providecommand{\cellmll}{\cellcolor[HTML]{FCF4F0}}
\providecommand{\cellmrr}{\cellcolor[HTML]{EEF4EC}}

\definecolor{generalcolor}{HTML}{C2E3EC}
\definecolor{specificcolor}{HTML}{DBEDC5}

\begin{longtable}{>{\centering\arraybackslash}m{4cm}>{\raggedright\arraybackslash}m{8cm}>{\centering\arraybackslash}m{3.0cm}}
\caption{PsyAlign: Comparative Ethical Framework for Counseling Professions and AI in Mental Health}\\
\toprule
\textbf{Principle Category (Counselor / AI)} & \centering\textbf{Content} & \textbf{Source} \\
\midrule
\endfirsthead
\multicolumn{3}{r}{\footnotesize\itshape{(Continued from previous page)}} \\
\toprule
\textbf{Principle Category (Counselor / AI)} & \centering\textbf{Content} & \textbf{Source} \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{\footnotesize\itshape{(Continued on next page)}} \\
\endfoot % End of page footer
\bottomrule
\endlastfoot
\midrule
\rowcolor{generalcolor}
\multicolumn{3}{c}{\textbf{COUNSELING PROFESSIONALS' ETHICAL PRINCIPLES}} \\
\midrule
\textbf{Non-Discrimination} & Psychologists shall treat service seekers justly and shall not discriminate against them based on age, gender, race, sexual orientation, religion, political affiliation, educational level, physical condition, or socioeconomic status. & \cite{psyethic_14_1} \\
\hline
\textbf{Confidentiality} & "Counselors do not share confidential information without client consent or without sound legal or ethical justification." & \cite{psyethic_14_2} \\
\hline
\textbf{Working with Minors} & When delivering counselling or therapy to children or minors, practitioners must ensure capacity to consent, involve caregivers/guardians appropriately, and act in the best interest of the child. & \cite{psyethic_14_4} \\
\hline
\textbf{Prohibition of Sexual Harassment} & Psychologists do not engage in sexual harassment. Sexual harassment is sexual solicitation, physical advances, or verbal or nonverbal conduct that is sexual in nature, that occurs in connection with the psychologist's activities or roles as a psychologist. & \cite{psyethic_14_5} \\
\hline
\textbf{Do No Harm} & Do no harm to people using our professional services, which includes avoiding actions that may cause physical, psychological, or emotional harm. & \cite{psyethic_14_6} \\
\hline
\textbf{Respect for Cultural Diversity} & Psychologists must respect the cultural diversity of service seekers. Psychologists should be fully aware of their own values and their potential influence on service seekers, respect the values of service seekers, and avoid imposing their own values on them or making important decisions on their behalf. & \cite{psyethic_14_1} \\
\hline
\textbf{Correcting Misconduct} & Psychologists, upon recognizing any misconduct or misunderstanding of their duties in their work, should take immediate measures to correct them. & \cite{psyethic_14_1} \\
\hline
\textbf{Referral Responsibility} & If a counselor lacks the competence to address a client's issues, or if the client is deriving minimal benefit from counseling, the counselor has a responsibility to assist the client in being referred to a more suitable professional. & \cite{psyethic_14_2, psyethic_14_5} \\
\hline
\textbf{Suicide/Homicide Risk Protocol} & Counselors must have explicit protocols for managing suicidal/homicidal ideation, including risk assessment, safety planning, and, when necessary, promptly notifying emergency contacts or authorities. & \cite{psyethic_14_2, psyethic_14_5} \\
\hline
\textbf{Evidence-Based Practice} & Counselors should only employ counseling techniques or therapeutic modalities that are supported by a scientific or professional evidence base. & \cite{psyethic_14_2} \\
\midrule
\rowcolor{specificcolor}
\multicolumn{3}{c}{\textbf{AI-SPECIFIC ETHICAL PRINCIPLES}} \\
\midrule
\textbf{Illusion of Authority} & AI systems should not create an inappropriate illusion of authority or expertise. & \cite{psyethic_14_3} \\
\hline
\textbf{Non-Medical Device Software} & Software that does not provide specific treatment or diagnosis recommendations is considered non–medical device software. & \cite{psyethic_14_7} \\
\hline
\textbf{Protection of Vulnerable Groups} & AI systems should include safeguards to protect vulnerable groups and individuals. & \cite{psyethic_14_8} \\
\hline
\textbf{Transparency of AI Identity} & AI systems should not be designed to mislead users into believing that they are engaging with a human being. & \cite{psyethic_14_9} \\
\bottomrule
\end{longtable}
